A general method for multiresolutional analysis of mesoscale features in dark-field x-ray microscopy images

Dark-field x-ray microscopy utilizes Bragg diffraction to collect full-field x-ray images of "mesoscale" structure of ordered materials. Information regarding the structural heterogeneities and their physical implications is gleaned through the quantitative analyses of these images. Namely, one must be able to extract diffraction features that arise from lattice modulations or inhomogeneities, quantify said features, and identify and track patterns in the relevant quantitative properties in subsequent images. Due to the necessity to track features with a wide array of shapes and length scales while maintaining spatial resolution, wavelet transforms were chosen as a potent signal analysis tool. In addition to addressing multiple length scales, this method can be used in conjunction with other signal processing methods such as image binarization for increased functionality. In this article, we demonstrate three effective use of wavelet analyses pertaining to DFXM. We show how to extract and track smooth linear features-which are diffraction manifestations of twin boundaries-as the sample orientation changes as it is rotated about momentum transfer. Secondly, we show that even the simplest wavelet transform, the Haar transform, can be used to capture the primary features in DFXM images, over a range of length scales in different regions of interest within a single image enabling localized reconstruction. As a final application, we extend these techniques to determine when a DFXM image is in focus.

==> scratch.tex <==
@book{lamport86,
  author = "Leslie Lamport",
  title  =  "{\LaTeX{}}: A Document Preparation System",
  publisher = {Addison-Wesley},
  year   = 1986                                           }

@article{pauling89,
  author = "L. Pauling",
  title  = {Icosahedral quasicrystals of intermetallic compounds are icosahedral twins of cubic crystals of three kinds, consisting of large (about 5000 atoms) icosahedral complexes in either a cubic body-centered or a cubic face-centered arrangement or smaller (about 1350 atoms) icosahedral complexes in the $\beta$-tungsten arrangement},
  journal = "Proc. Natl Acad. Sci USA",
  volume = 86,
  pages  = "8595--8599",
  year   = 1989                                           }

@article{zahir,
  author = "Z. Qiao and Z. Islam",
  title  =  "A large field-of-view high-resolution hard x-ray microscope using polymer optics",
  journal = "Review of Scientific Instruments 91",
  volume = "91",
  doi    = "10.1063/5.0011961",
  year   = 2020                                           }


@misc{dresselhaus,
  doi = "10.48550/ARXIV.2008.04972",
  
  url = "https://arxiv.org/abs/2008.04972",
  
  author = "A. Gonzalez",
  
  keywords = "Data Analysis, Statistics and Probability (physics.data-an), Image and Video Processing (eess.IV), FOS: Physical sciences, FOS: Physical sciences, FOS: Electrical engineering, electronic engineering, information engineering, FOS: Electrical engineering, electronic engineering, information engineering",
  
  title = "Methods to Quantify Dislocation Behavior with Dark-field X-ray Microscopy Timescans of Single-Crystal Aluminum",
  
  publisher = "arXiv",
  
  year = 2020,
  
  copyright = "arXiv.org perpetual, non-exclusive license"
}

@misc{tamraz,
  
  
  author = "R. Tamraz",
  
  title = {Intelligent optical imaging to steer and enhance high-resolution dark-field x-ray microscopy at the Advanced Photon Source},
  
  year = 2021,
  
}

@article{melt
doi:10.1126/sciadv.abe8311,
author = {Leora E. Dresselhaus-Marais  and Grethe Winther  and Marylesa Howard  and Arnulfo Gonzalez  and Sean R. Breckling  and Can Yildirim  and Philip K. Cook  and Mustafacan Kutsal  and Hugh Simons  and Carsten Detlefs  and Jon H. Eggert  and Henning Friis Poulsen },
title = {In situ visualization of long-range defect interactions at the edge of melting},
journal = {Science Advances},
volume = {7},
number = {29},
pages = {eabe8311},
year = {2021},
doi = {10.1126/sciadv.abe8311},
URL = {https://www.science.org/doi/abs/10.1126/sciadv.abe8311},
eprint = {https://www.science.org/doi/pdf/10.1126/sciadv.abe8311},
abstract = {Dark-field X-ray microscopy movies reveal how patterns of microscopic defects in bulk aluminum destabilize from 97-99\% of melting. Connecting a bulk material’s microscopic defects to its macroscopic properties is an age-old problem in materials science. Long-range interactions between dislocations (line defects) are known to play a key role in how materials deform or melt, but we lack the tools to connect these dynamics to the macroscopic properties. We introduce time-resolved dark-field x-ray microscopy to directly visualize how dislocations move and interact over hundreds of micrometers deep inside bulk aluminum. With real-time movies, we reveal the thermally activated motion and interactions of dislocations that comprise a boundary and show how weakened binding forces destabilize the structure at 99\% of the melting temperature. Connecting dynamics of the microstructure to its stability, we provide important opportunities to guide and validate multiscale models that are yet untested.}}


\begin{comment}
\begin{references}

\bibitem{Melt} L.E. Dresselhaus-Marais, G. Winther, M. Howard, A. Gonzalez, S.R. Breckling, C. Yildirim, P.K. Cook, et al. \textit{In Situ Visualization of Long-Range Defect Interactions at the Edge of Melting}, \textit{Science Advances} 7, no. 29 (July 16, 2021). https://doi.org/10.1126/sciadv.abe8311.
\bibitem{Ahl} S.R. Ahl, \textit{Elements of a Method for Multiscale Characterization of Recrystallization in Deformed Metals}, Department of Physics, Technical University of Denmark (2018).
\bibitem{swt} G. Nason and B. Silverman, \textit{The Stationary Wavelet Transform and Some Statistical Applications} (1995).
\bibitem{Rosenberg} H.M. Rosenberg, \textit{The Solid State: An Introduction to Physics of Solids for Students of Physics, Material Science and Engineering}. Oxford U.P, Oxford 1988.
\bibitem{Ashcroft} N.W. Ashcroft and N.D. Mermin, \textit{Solid State Physics} (Saunders College, Fort Worth, 1988).
\bibitem{wavelet} J.S. Walker, \textit{A Primer on Wavelets and Their Scientific Applications} (Chapman & Hall, Boca Raton, Fla., 2008).
\bibitem{MatIm} O. Marques, \textit{Practical Image and Video Processing Using MATLAB} (J. Wiley & Sons/IEEE Press, Hoboken, N.J., 2011).
\bibitem{Matlab} ``Matlab," https://www.mathworks.com/products/matlab.html. 

\end{references}
\end{comment}
